Automatic and Efficient Variability-Aware Lifting of Functional Programs

A software analysis is a computer program that takes some representation of a software product as input and produces some useful information about that product as output. A software product line encompasses \emph{many} software product variants, and thus existing analyses can be applied to each of the product variations individually, but not to the entire product line as a whole. Enumerating all product variants and analyzing them one by one is usually intractable due to the combinatorial explosion of the number of product variants with respect to product line features. Several software analyses (e.g., type checkers, model checkers, data flow analyses) have been redesigned/re-implemented to support variability. This usually requires a lot of time and effort, and the variability-aware version of the analysis might have new errors/bugs that do not exist in the original one. Given an analysis program written in a functional language based on PCF, in this paper we present two approaches to transforming (lifting) it into a semantically equivalent variability-aware analysis. A light-weight approach (referred to as \emph{shallow lifting}) wraps the analysis program into a variability-aware version, exploring all combinations of its input arguments. Deep lifting, on the other hand, is a program rewriting mechanism where the syntactic constructs of the input program are rewritten into their variability-aware counterparts. Compositionally this results in an efficient program semantically equivalent to the input program, modulo variability. We present the correctness criteria for functional program lifting, together with correctness proof sketches of our program transformations. We evaluate our approach on a set of program analyses applied to the BusyBox C-language product line.

==> motivation.tex <==
\section{Motivation}
\label{sec:motivation}

% introducing SPLs
This work is primarily motivated by the need of software analyses to intrinsically handle variability within an SPL. An SPL is a family of software products sharing some functionalities, but also different products within the family can exhibit different features. The benefit of following an SPL approach (as opposed to building each product separately) is that the artifacts contributing to the common behavior are shared across the product line. This saves the time and effort that would have been otherwise wasted re-engineering the same artifacts for each of the product family members.

% fig:annotative - an example of an annotative SPL
\begin{figure}
\begin{multicols}{2}
\begin{minted}[linenos]{cpp}
int foo

#ifdef A
  (int a) {
#ifdef B
    return a * 2;
#else
    return a * 3 + 1;
#endif

#else // !A
  (int a, int b) {
    return (a  
#ifdef B
	+
#else
	* 2 +
#endif
	b);
#endif

}
\end{minted}

\columnbreak

\begin{minted}{cpp}
// A /\ B
int foo
  (int a) {
    return a * 2;
}

// A /\ !B
int foo
  (int a) {
    return a * 3 + 1;
}

// !A /\ B
int foo
  (int a, int b) {
    return (a + b);
}

// !A /\ !B
int foo
  (int a) {
    return (a * 2 + b);
}
\end{minted}

\end{multicols}
\caption{Example of an annotative product line, with the \onefifty~on the left-hand side, and the four products that can be generated from it on the right-hand side.}
\label{fig:annotative}
\end{figure}
% end - fig:annotative

% explaining variability in the context of SPLs
The differences in behavior between different members of the product family (different product variants) are explicitly specified within the different SPL artifacts (source code, models, test cases, etc...). There are different approaches to specifying these differences. In this paper we only cover the \tm{annotative}~\cite{Czarnecki:Antkiewicz:2005,Kastner:Apel:2008,rubin12} approach, where an individual construct can be annotated with an expression indicating the set of product variants to which that construct belongs. 

Fig.~\ref{fig:annotative} shows a very simple example of a \tm{Software Product Line (SPL)} $P$ written in the C language, where C Pre-Processor (CPP) conditional compilation macros are used to associate different syntactic constructs to different features. This collective representation of the whole SPL (not just the artifacts of a single product) is usually referred to as the \onefifty~of the SPL.

The different code snippets within \emph{\#ifdef}-\emph{\#endif} blocks are only present when the \emph{\#ifdef} expression is true. By setting/unsetting different macros, these expressions can either evaluate to true or false, and thus at preprocessing time we can vary the code constructs that actually get compiled. When each of those macros correspond to a program feature, the CPP becomes a tool for enabling/disabling individual features.

It is worth mentioning that the CPP allows for encapsulating arbitrary sequences of syntactic tokens within \emph{\#ifdef} blocks. Those sequences by themselves do not need to be syntactically correct. However, when embedded into the rest of the program as a part of preprocessing, the result needs to be syntactically correct for the program to compile. For example, snippets in lines 16 and 18 are not syntactically correct by themselves, but when spliced with line 14 the resultant expression (whether \FB is included or not) is syntactically correct.

% introducing software analyses
Pretty much like all software products, the process of engineering and maintaining SPLs involves the use of many analysis tools. These tools range from syntax checkers (parsers) to model checkers and other bug finding tools. Many analysis tools have been developed over the years, and many of them are already incorporated into development toolchains. Those tools work on products though, not on product lines. 

% explaining the intractability of brute force SPL analysis
For SPL engineers, using any of the existing analysis tools would require generating a single product from the product line and applying the tool to it. To apply the tool to the whole product line, each individual product needs to be generated and have the tool applied to. Since many of the SPL features can be combined with others, the number of possible products grows exponentially with the number of features. As a result, enumerating all products, let alone analyzing each of them, is practically intractable. 

% explaining the tediousness of manually rewriting analyses for SPLs
To get around the intractability of analyzing each possible product, some product sampling techniques have been suggested~\cite{Apel:2013,Liebig:2013}. Sampling tackles the combinatorial complexity of the problem by giving up completeness. To mitigate that, several analyses have been rewritten to support full SPL analysis. This includes syntax checkers (parsers)~\cite{Kastner:2011,Gazzillo:2012}, type checkers~\cite{Kastner:2012}, model checkers~\cite{Classen:2013}, data-flow analyses~\cite{Bodden:2013}, and abstract interpretation analyses~\cite{Midtgaard:2015}. Although the high level algorithm is the same as that of the single product analysis, re-developing each of these analyses from scratch is tedious, time consuming and potentially error prone. 

% highlighting the fact that when analyzing an SPL, many of the intermediate calculations are common across different variants and do not need to be recalculated
The SPL analysis algorithm in all these cases is the same as the single product analysis applied to different construct variants, while maximizing the reuse of intermediate results computed from common constructs. For example, if a C function that is a 100 lines of code has only two lines of code annotated with \emph{\#ifdef} directives, then we have almost 98\% of the function common across all variants. Any analysis applied to this function will typically compute many intermediate values that are independent of the varying two lines of code. Those values are essentially shared across different variants, and they do not need to be recomputed over and over. An efficient SPL analysis has to maximize the utilization of those common computations, and minimize the number of variant-specific computations.

% lifting TLC analyses
Since analyses are essentially computer programs taking software artifacts as input, and since the algorithms implemented by these programs need to be preserved in the SPL version, the question we are trying to answer is whether these programs can be automatically rewritten into versions that support SPLs. To avoid tackling the problem only for analyses written in a specific programming language, we wanted to use a generic program formalism. Typed Lambda Calculus (TLC) serves that purpose by being both simple compared to higher level programming languages, and still as expressive as any other language due to its Turing completeness.




==> rewriting.tex <==
\section{Rewriting Algorithm}
\label{sec:rewriting}

Given an TLC program (a non-empty set of functions), the program is rewritten into a lifted program satisfying the correctness condition using Algorithm~\ref{alg:rewriting}. This algorithm is syntax-directed, traversing the Abstract Syntax Tree (AST) of the program and rewriting each construct, while maintaining the syntactic validity of the resulting program. 

\begin{algorithm}
\caption{Rewriting algorithm}
\label{alg:rewriting}

\begin{algorithmic}[1]

\Procedure{RewriteFunction}{$\term{f}, \term{fs}$}		\Comment{return a deep-lifted version of a function f}
\ForAll{$\term{n}$ in nodes($\term{f}$)}	\Comment{traverse the AST of f}

\If{$\term{n}$ is Variable}		
\State{$t \gets (\term{liftT}~\term{n})$}
\ElsIf{$\term{n}$ is Abstraction}
\State{$t \gets$ RewriteFunction(n)}
\Else		\Comment{$\term{n}$ is Application}

\If{$\term{n} \in \term{fs}$}
	\State{$t \gets n'$}	\Comment{use the deep-lifted function}
\Else		\Comment{apply the shallow-lifted function}
	\State{$t \gets (\term{apply} (\term{liftT}~n))$}
\EndIf

\EndIf

\State{Write t}

\EndFor
\EndProcedure

\Procedure{Rewrite}{$\term{fs}$} \Comment{Rewrite the set of functions fs into lifted versions}
\ForAll{$f$ in $\term{fs}$}
\State $f' \gets$ RewriteFunction(f)
\EndFor
\EndProcedure

\end{algorithmic}

\end{algorithm}

The rewriting algorithm makes a single pass through the AST of the input program. In TLC programs, each node will be either a variable, a lambda abstraction or a lambda application. A variable is rewritten with a lifted variable with the $\top$ presence condition using the \textbf{liftT} operator (line 4). A lambda abstraction is recursively rewritten into a lifted version (line 6). 

For lambda applications, we need to distinguish between applying functions that we are rewriting (referred to as \tm{deep-lifted functions} and calling other functions (what we call \tm{shallow-lifted functions}). This distinction is necessary because external library function or primitive operators (e.g., equality comparison, addition) will not be rewritten, and will be used as a black box by the \textbf{apply} combinator.

The \textbf{Rewrite} procedure iterates over all the functions that are to be rewritten, and for each calls the \textbf{RewriteFunction} procedure.

The time complexity of the algorithm is $O(n)$, where $n$ is the number of nodes in the AST.
